SFD2: Semantic-guided Feature Detection and Description

Visual localization is a fundamental task for various applications including autonomous driving and robotics. Prior methods focus on extracting large amounts of often redundant locally reliable features, resulting in limited efficiency and accuracy, especially in large-scale environments under challenging conditions. Instead, we propose to extract globally reliable features by implicitly embedding high-level semantics into both the detection and description processes. Specifically, our semantic-aware detector is able to detect keypoints from reliable regions (e.g. building, traffic lane) and suppress unreliable areas (e.g. sky, car) implicitly instead of relying on explicit semantic labels. This boosts the accuracy of keypoint matching by reducing the number of features sensitive to appearance changes and avoiding the need of additional segmentation networks at test time. Moreover, our descriptors are augmented with semantics and have stronger discriminative ability, providing more inliers at test time. Particularly, experiments on long-term large-scale visual localization Aachen Day-Night and RobotCar-Seasons datasets demonstrate that our model outperforms previous local features and gives competitive accuracy to advanced matchers but is about 2 and 3 times faster when using 2k and 4k keypoints, respectively.

==> figs_tables/fig_hpatches.tex <==
\setlength{\tabcolsep}{1.5pt}
\begin{figure*}[t]
	%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
	\centering
	\begin{minipage}{0.5\linewidth}
		\centerline{\includegraphics[width=1.\linewidth]{images/exp/hseq}}
	\end{minipage}
	\begin{minipage}{0.45\linewidth}
		%\footnotesize
		%\scriptsize
		\tiny
		\begin{threeparttable}
			\begin{tabular}{lccl}
				\toprule
				Methods & \#Features & \#Match & \#D\\
				\midrule
				HesAff + RootSIFT~\cite{hessian, rootsift} & 6.7K & 2.8K & 128\\
				HAN + HN++~\cite{hardnet} & 3.9K & 2.0K & 128\\
				LF-Net~\cite{lfnet} & 0.5K & 0.2K & 256\\
				SuperPoint~\cite{superpoint} & 1.7K & 0.9K & 256\\
				DELF~\cite{delf2017} & 4.6K & 1.9K & 128\\
				D2-Net~\cite{d2-net} & 8.3K & 2.8K & 512\\
				R2D2~\cite{r2d2} & 5.0K & 1.8K & 128\\
				DISK~\cite{disk} & 8.2k & 4.0k & 128 \\
				CAPS + SIFT~\cite{caps} & 4.4K & 1.5K & 256\\
				%Caps w/ SuperPoint & 1.7K & 0.9K \\
				Ours (D=128) & 3.7K & 1.3K & 128\\  
				Ours (D=32) & 3.5K & 1.2K & 32\\
				\bottomrule
			\end{tabular}
		\end{threeparttable}
	\end{minipage}

	\caption{\textbf{Mean matching accuracy (MMA) on HPatches~\cite{hpatches}}. We show the MMA at different error thresholds. On the right side, the number of detected keypoints and mutual nearest matches are also listed. Our method performs consistently better than previous systems in terms of illumination and viewpoint changes. Our descriptors with size of 32 give close accuracy as R2D2~\cite{r2d2} when the error threshold is less than 6px.}
	\label{fig:hpatches}
\end{figure*}

==> figs_tables/fig_hpatches_ext.tex <==
\setlength{\tabcolsep}{1.5pt}
\begin{figure*}[t]
	%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
	\centering
	\begin{minipage}{0.6\linewidth}
		\centerline{\includegraphics[width=1.\linewidth]{images/exp/hseq_full}}
	\end{minipage}
	\begin{minipage}{0.35\linewidth}
		%\footnotesize
		%\scriptsize
		\tiny
		\begin{threeparttable}
			\begin{tabular}{lcccccl}
				\toprule
				Methods & \#Features & \#Match & Illu.@5px & Viewp.@5px & All@5px & \#D\\
				\midrule
				HesAff + RootSIFT~\cite{hessian, rootsift} & 6.7K & 2.8K & 0.587 & 0.690 & 0.641 &128\\
				HAN + HN++~\cite{hardnet} & 3.9K & 2.0K & 0.697 & 0.709 & 0.703 &128\\
				DELF~\cite{delf2017} & 4.6K & 1.9K & 0.903 & 0.275 & 0.577 &128\\
				SuperPoint~\cite{superpoint} & 1.7K & 0.9K & 0.782 & 0.679 & 0.729 &256\\
				LF-Net~\cite{lfnet} & 0.5K & 0.2K & 0.620 &  0.527 & 0.572 &256\\
				D2-Net~\cite{d2-net} & 8.3K & 2.8K & 0.640 &  0.553 & 0.595 &512\\
				R2D2~\cite{r2d2} & 5.0K & 1.8K & 0.887 & 0.773 & 0.828 & 128\\
				CAPS + SIFT~\cite{caps} & 4.4K & 1.5K & 0.842 & 0.737 & 0.789 &256\\
				ContextDesc~\cite{contextdesc} & 4.0k & 1.7k & 0.659 & 0.715 & 0.688 & 128 \\
				ASLFeat~\cite{aslfeat} & 4.0k & 2.0k & 0.878 & 0.769 & 0.821 & 128\\ 
				ASLFeat~\cite{aslfeat} & 4.8k & 2.1k & 0.864 & 0.793 & 0.828 & 128\\ 
				DISK (8k)~\cite{disk} & 8.2k & 4.0k & 0.917 & 0.797 & 0.855 &128 \\
				DISK (2k)~\cite{disk} & 2.0k & 1.0k & 0.897 & 0.759 & 0.826 & 128 \\
				%Caps w/ SuperPoint & 1.7K & 0.9K \\
				Ours (128) & 3.7K & 1.3K & \textbf{0.920} & \textbf{0.816} & \textbf{0.865} & 128\\  
				Ours (32) & 3.5K & 1.2K & 0.842 & 0.755 & 0.797 & 32\\
				\bottomrule
			\end{tabular}
		\end{threeparttable}
	\end{minipage}

	\caption{\textbf{Mean matching accuracy (MMA) on HPatches~\cite{hpatches}}. We show the MMA at different error thresholds. On the right side, the number of detected keypoints, mutual nearest matches, and size of descriptors are also listed. The best results are highlighted.}
	\label{fig:hpatches}
	%Our method performs consistently better than previous systems in terms of illumination and viewpoint changes. Our descriptors with size of 32 give close accuracy as R2D2~\cite{r2d2} when the error threshold is less than 6px. 
\end{figure*}

==> figs_tables/table_dataset.tex <==
\setlength{\tabcolsep}{1.pt}

\begin{table}
		\footnotesize
	%\small
	\centering
	\begin{threeparttable}
		\begin{tabular}{lcccccc}
			\toprule
			Dataset & Reference & Query & Day & Night & Seasons & Semantics \\
			\toprule
			Aachen\_v1.1 & 6,697 & 1015 & \cmark & \cmark & \cmark & building, road, tree\\
			RCS & 16,121 & 11,934 & \cmark & \cmark & \cmark & building, road, tree\\
			ECS & 60,937 & 56,613 & \cmark & & \cmark & road, tree\\
			\bottomrule
		\end{tabular}
	\end{threeparttable}
\caption{Some examples and their categories. All objects are categorized into four groups denoted as \textit{Volatile}, \textit{Dynamic}, \textit{Short-term}, and \textit{Long-term} according to the their properties. Different categories are assigned with cascade experienced \textit{Stability} values.}

\label{tab:dataset}
\end{table}

==> figs_tables/table_ecmu_4.tex <==
\setlength{\tabcolsep}{0.8pt}

\begin{table}
	%\footnotesize
	%\tiny
	\scriptsize
	\centering
	\begin{center}
		\begin{tabular}{lcccl}
			Method & urban & suburban & overcast  & cloudy  \\
			%\hline
			%\hline
			\toprule
			NV~\cite{netvlad} & 12.2 / 31.5 / 89.8 & 3.7 / 13.9 / 74.7  & 6.7 / 19.1 / 76.3 &  6.8 / 20.1 / 79.5  \\
			DV~\cite{densevlad} & 14.7 / 36.3 / 83.9 & 5.3 / 18.7 / 73.9 & 8.4 / 23.3 / 72.1  &  9.3 / 27.3 / 80.5 \\
			AS~\cite{as} & 81.0 / 87.3 / 92.4 & 62.6 / 70.9 / 81.0 & 64.1 / 70.8 / 78.6 & 71.6 / 77.6 / 84.2 \\
			AHM~\cite{ahm2019} & 65.7 / 82.7 / 91.0 & 66.5 / 82.6 / 92.9 & 62.8 / 78.8 / 89.4 & 69.4 / 84.4 / 92.8 \\
			CSL~\cite{csl} & 71.2 / 74.6 / 78.7 & 57.8 / 61.7 / 67.5 & 52.2 / 55.4 / 60.3 & 63.3 / 66.3 / 70.5 \\
			FGSN~\cite{fgsn} & 85.3 / 91.0 / 94.6 & 69.5 / 76.4 / 83.7 & 70.5 / 77.1 / 83.4  & 77.8 / 82.9 / 87.5 \\
			% +SSMC
			GSMC~\cite{gsmc} & 86.4 / 91.2 / 93.8 & 77.0 / 82.9 / 88.7 & 69.9 / 75.0 / 79.6 & 76.2 / 79.8 / 83.0  \\
			%-200
			SP~\cite{superpoint} & 89.6 / 95.1 / 97.4 & 75.3 / 82.5 / 89.5 & 77.8 / 84.7 / 90.6 & 82.0 / 88.1 / 92.5\\
			R2D2~\cite{r2d2} & 89.7 / 96.6 / 98.3 & 76.1 / 83.8 / 89.0 & 79.9 / 87.0 / 90.6 & 84.1 / 90.0 / 92.5\\
			Ours & 90.2 / 96.7 / 98.2 & 76.9 / 84.5 / 89.3 & 81.6 / 88.5 / 91.4 &  84.6 / 90.7 / 93.0\\
			\bottomrule
		\end{tabular}
	\end{center}
\caption{Localization accuracy on the Extended-CMU-Seasons dataset. We report the percentages of successfully localized images within 3 error thresholds ($0.5m,2^\circ$, $1m,5^\circ$, and $5m,10^\circ$)}.
\end{table}

==> figs_tables/table_ecmu_full.tex <==
\setlength{\tabcolsep}{1pt}

\begin{table*}
	%\footnotesize
	\tiny
	\centering
	\begin{center}
		\begin{tabular}{cccccccccccc}
			Method & urban & suburban & park & overcast & sunny & foliage & mixed foliage & no foliage & low sun & cloudy & snow \\
			%\hline
			%\hline
			\toprule
			NetVlad~\cite{netvlad} & 12.2/31.5/89.8 & 3.7/13.9/74.7 & 2.6/10.4/55.9 & 6.7/19.1/76.3 & 6.4/18.8/73.2  & 6.2/18.5/74.3 & 5.8/17.6/71.1 & 6.7/20.9/79.4 & 5.5/17.5/71.3	& 6.8/20.1/79.5 & 5.0/16.4/68.0 \\
			DenseVlad~\cite{densevlad} & 14.7/36.3/83.9 & 5.3/18.7/73.9 & 5.2/19.1/62.0 & 8.4/23.3/72.1 & 7.6/21.3/66.8 & 7.4/21.1/68.0 & 8.5/24.5/73.0 & 10.0/32.6/88.0 & 8.3/26.1/76.0 & 9.3/27.3/80.5 & 8.3/29.0/78.9\\
			AS~\cite{as} & 81.0/87.3/92.4 & 62.6/70.9/81.0 & 45.5/51.6/62.0 & 64.1/70.8/78.6 & 55.2/62.3/71.3 & 58.8/65.3/73.9 & 59.2/67.5/77.4 & 83.3/88.9/94.6 & 65.8/73.4/82.8 & 71.6/77.6/84.2 & 73.0/81.0/90.5\\
			CSL~\cite{csl} & 71.2/74.6/78.7 & 57.8/61.7/67.5 & 34.5/37.0/42.2 & 52.2/55.4/60.3 & 43.3/46.6/51.9 & 47.0/50.2/55.3 & 52.4/56.1/62.0 & 80.3/83.2/86.6 & 61.7/65.3/70.7 & 63.3/66.3 /70.5 & 69.9/73.7/78.7\\
			FGSN+SSMC~\cite{fgsn} & 85.3/91.0/94.6 & 69.5/76.4/83.7 & 51.4/57.6/65.5 & 70.5/77.1/83.4 & 61.9/68.4/74.9 & 65.5/71.6/77.7 & 66.0/73.3/81.0 & 84.6/89.6/93.5 & 70.5/77.0/84.0 & 77.8/82.9/87.5 & 74.2/81.5/88.2 \\
			GSMC-200~\cite{gsmc} & 86.4/91.2/93.8 & 77.0/82.9/88.7 & 38.9/43.4/50.0 & 69.9/75.0/79.6 & 59.4/64.9/70.3 & 64.3/69.4/74.4 & 65.0/70.7/76.6 & 87.2/91.0/94.3 & 72.2/77.7/83.3 & 76.2/79.8/83.0 & 79.7/85.4/91.0 \\
			SP-NV~\cite{superpoint} & 89.6/95.1/97.4 & 75.3/82.5/89.5 & 61.7/69.1/78.4 & 77.8/84.7/90.6 & 67.6/75.5/84.5 & 70.9/78.3/86.3 & 75.6/82.5/88.5 & 88.5/93.1/95.3 & 78.7/84.7/89.7 & 82.0/88.1/92.5 & 82.0/87.1/90.9 \\
			R2D2-NV~\cite{r2d2} & 89.7/96.6/98.3 & 76.1/83.8/89.0 & 64.4/72.1/76.5 & 79.9/87.0/90.6 & 70.3/78.3/83.2 & 74.1/81.2/85.6 & 75.7/84.1/87.9 & 86.6/93.3/95.3 & 77.8/85.7/89.3 & 84.1/90.0/92.5 & 79.8/87.6/91.1\\
			Ours & 90.2/96.7/98.2 & 76.9/84.5/89.3 & 65.4/73.1/77.0 & 81.6/88.5/91.4 & 70.0/78.2/83.1 & 74.2/81.5/85.8 & 77.5/85.3/88.6 & 87.1/93.2/95.1 & 79.2/86.4/89.6 & 84.6/90.7/93.0 & 80.3/87.5/90.6\\
			\bottomrule
		\end{tabular}
	\end{center}
\caption{Localization accuracy on the Extended-CMU-Seasons dataset. We report the percentages of successfully localized images within 3 error thresholds ($0.5m,2^\circ$, $1m,5^\circ$, and $5m,10^\circ$)}.
\end{table*}

==> figs_tables/table_ecmu_v2.tex <==
\setlength{\tabcolsep}{4.pt}

\begin{table}
	%\footnotesize
	%\tiny
	\scriptsize
	\centering
		\begin{tabular}{lccc}
			\toprule
			Method & urban & suburban & cloudy   \\
			%\hline
			%\hline
			\midrule
			%NV~\cite{netvlad} & 12.2 / 31.5 / 89.8 & 3.7 / 13.9 / 74.7  & 6.7 / 19.1 / 76.3  \\
			%DV~\cite{densevlad} & 14.7 / 36.3 / 83.9 & 5.3 / 18.7 / 73.9 & 8.4 / 23.3 / 72.1  \\
			AS~\cite{as} & 81.0 / 87.3 / 92.4 & 62.6 / 70.9 / 81.0 & 71.6 / 77.6 / 84.2 \\
			%AHM~\cite{ahm2019} & 65.7 / 82.7 / 91.0 & 66.5 / 82.6 / 92.9 & 62.8 / 78.8 / 89.4 \\
			CSL~\cite{csl} & 71.2 / 74.6 / 78.7 & 57.8 / 61.7 / 67.5 & 63.3 / 66.3 / 70.5  \\
			\midrule
			LLN~\cite{lln} & 84.3 / 89.3 / 93.0	& 68.0 / 75.1 / 84.4 & 73.1 / 78.7 / 86.2 \\
			FGSN~\cite{fgsn} & 85.3 / 91.0 / 94.6 & 69.5 / 76.4 / 83.7 & 77.8 / 82.9 / 87.5 \\
			% +SSMC
			SMC~\cite{smc} & 86.4 / 91.2 / 93.8 & 77.0 / 82.9 / 88.7 & 76.2 / 79.8 / 83.0  \\
			SSM~\cite{ssm} & 88.8 / 93.6 / 96.3 & \textbf{78.0} / 83.8 / 89.2 & \textbf{86.4} / 90.5 / 92.9\\
			DASGIL-FD~\cite{dasgil} & 17.4 / 42.0 / 91.1 & 6.7 / 22.1 / 88.5 & 10.0 / 28.9 / 92.1 \\
			%-200
			\midrule
			SIFT~\cite{sift} & 56.9 / 63.9 / 70.2 & 37.8 / 45.3 / 55.4 & 43.0 / 49.6 / 58.3 \\
			SPP~\cite{superpoint} & 89.6 / 95.1 / 97.4 & 75.3 / 82.5 / 89.5 & 77.8 / 84.7 / 90.6 \\
			D2-Net~\cite{d2-net} & 82.6 / 94.8 / 98.4 & 75.9 / \textbf{86.8} / \textbf{93.8} & 82.0 / 88.1 / 92.5 \\
			R2D2~\cite{r2d2} & 89.7 / 96.6 / 98.3 & 76.1 / 83.8 / 89.0 & 84.1 / 90.0 / 92.5 \\
			%Ours (128) & \textbf{90.2} / \textbf{96.7} / 98.2 & \textbf{76.9} / \textbf{84.5} / \textbf{89.3} & \textbf{81.6} / \textbf{88.5} / \textbf{91.4} \\
			\midrule
			Ours (128) & \textbf{90.3} / \textbf{97.1} / \textbf{98.5} & 77.9 / 85.6 / 90.4 & 84.9 / \textbf{91.1} / \textbf{93.4} \\
			Ours (32) & 88.9 / 95.8 / 97.7 & 73.2 / 80.7 / 87.2 & 80.8 / 87.3 / 90.7 \\
			\bottomrule
		\end{tabular}
\caption{\textbf{Localization accuracy on the Extended-CMU-Seasons dataset.} The best results are highlighted. }.
\label{tab:ecmu}
\end{table}

==> figs_tables/table_hpatches.tex <==
\setlength{\tabcolsep}{4.pt}

\begin{table}
	%\footnotesize
	%\small
	\scriptsize
	\centering
	\begin{threeparttable}
		\begin{tabular}{lccc}
			\toprule 
			Methods & $\epsilon$ = 1 & $\epsilon$ = 3 & $\epsilon$ = 5 \\
			\midrule 
			SIFT~\cite{sift} & 40.5 & 68.1 & 77.6 \\
			LF-Net~\cite{lfnet} & 34.8 & 62.9 & 73.8 \\
			SuperPoint~\cite{superpoint} & 37.4 & 73.1 & 82.8 \\
			D2-Net~\cite{d2-net} & 16.7 & 61.0 & 75.9 \\
			R2D2~\cite{r2d2} & 39.1 & 75.7 & 85.7 \\
			DISK~\cite{disk} & 36.5 & 73.0 & 83.2 \\
			ASLFeat (MS)~\cite{aslfeat} & 35.6 & 69.3 & 82.6 \\
			\midrule
			ContextDesc~\cite{contextdesc} & 41.0 & 73.1 & 82.2 \\
			CAPS + SIFT~\cite{caps, sift} & 34.6 & 72.2 & 81.7 \\
			CAPS + SuperPoint~\cite{caps, superpoint} & \textbf{44.8} & 74.5 & 85.7\\
			\midrule
			Ours (128) & 43.5 & \textbf{77.8} & \textbf{86.3} \\
			Ours (32) & 43.5 & 76.1 & 85.9 \\
			\bottomrule 
 		\end{tabular}
 	\end{threeparttable}

\caption{\textbf{Success ratio of homography estimation on HPatches~\cite{hpatches}.} We extract 1k keypoints for all methods and report the success ratio with error thresholds of 1, 3, 5 pixels.}

  \label{tab:homography}
\end{table}

==> figs_tables/table_hpatches_sfm.tex <==
\setlength{\tabcolsep}{4.pt}

\begin{table}
		\footnotesize
	%\small
	\centering
	\begin{center}
		\begin{tabular}{cc|c}
			& \multicolumn{2}{c}{\textbf{HPatches}} \\
			& Rep. & MLE \\
			\hline
			DoG~\cite{sift} & 0.438 & 1.00 \\
			\hline
			Harris~\cite{harris} & 0.531 & 1.18 \\
			\hline
			SuperPoint~\cite{superpoint} & 0.496 & 1.04 \\ 
			\hline
			HF-Net~\cite{hfnet} & 0.466 & 1.14 \\
			D2-Net~\cite{d2-net} & 1 & 1 \\
			\hline
			R2D2~\cite{r2d2} & 1 & 1 \\
		\end{tabular}
	\end{center}
\caption{\textbf{Evaluation on the keypoint detectors.} The repeatability (Rep.) and mean localization error (MLE) are reported on the HPatches dataset~\cite{hpatches}.}
\end{table}

==> figs_tables/table_map.tex <==
\setlength{\tabcolsep}{4.pt}

\begin{table}
	%\footnotesize
	%\small
	\scriptsize
	\centering
	\begin{tabular}{lccccc}
		\toprule
		Method &  Repoj. error & \#Track length & \#Obs & \#3D points & Map size \\
		\midrule 
		SIFT~\cite{sift} & 0.9 & 5.6 & 1.2K & 1.4M & 3.8G\\
		SPP~\cite{superpoint} & 1.4 & 5.7 & 1.4K & 1.6M & 8.9G \\
		CAPS~\cite{caps} & 1.4 & 5.3 & 1.3K & 1.7M & 8.3G\\
		D2-Net~\cite{d2-net} & 1.6 & 3.7 & 1.2K & 2.2M & 15.3G\\
		R2D2~\cite{r2d2} & 1.3 & 8.3 & 1.7K & 1.3M & 5.4G\\
		ASLFeat~\cite{aslfeat} & 1.3 & 6.2 & 2.0k & 2.2M & 6.3G\\
		\midrule
		Ours (128) & 1.3 & 8.9 & 1.8K & 1.3M & 5.7G\\
		Ours (32) & 1.2 & 8.7 & 1.7K & 1.3M & 1.4G\\
		Ours (32, float16) & 1.2 & 8.7 & 1.7K & 1.3M & 0.7G\\
		\bottomrule 
	\end{tabular}
% & $0.5m,2^\circ$& $1m,5^\circ$& $5m,10^\circ$
\caption{\textbf{Details of 3D map.} We report the mean value of reprojection error (pixel), tracking length, number of observations and the total number of valid 3D points and the map size. }
\label{tab:map}
\end{table}

==> figs_tables/table_network.tex <==
\setlength{\tabcolsep}{4.pt}

\begin{table}[t]
	%\footnotesize
	\small
	\centering
	\begin{threeparttable}
		\begin{tabular}{lc}
			\toprule
			Layer Name & $C_{i}$, $C_{o}$, $k$, $s$, $d$, $p$ \\
			\midrule
			Input & 3, -, -, -, -, - \\ 
			Layer1 & 3, 64, 3, 1, 1, 1\\
			Layer2 & 64, 64, 3, 2, 1, 1\\
			Layer3 & 64, 128, 3, 1, 1, 1\\
			Layer4 & 128, 128, 3, 2, 1, 1\\
			Layer5 & 24, 32, 3, 1, 1, 1\\
			Layer6 & 32, 32, 3, 1, 1, 1\\
			Layer7 & 32, 64, 3, 1, 1, 1\\
			Layer8 & 64, 64, 3, 1, 2, 2\\
			Layer9 & 64, 128, 3, 1, 2, 2\\
			Layer10 & 128, 128, 3, 1, 4, 4\\
			Layer11 & 128, 128, 2, 1, 2, 4\\
			Layer10 & 128, 128, 2, 1, 4, 8\\
			Layer10 & 128, 128, 2, 1, 8, 16\\
			Descriptor Head  & 128, 128, 1, 1, 1, 0\\
			Detector Head & 128, 1, 1, 1, 1, 0\\
		
			
			\bottomrule
		\end{tabular}
	\end{threeparttable}
\caption{\textbf{Details of the network}. Following R2D2~\cite{r2d2}, we adopt the L2Net~\cite{l2-net} as the backbone. Details of input channel $C_{in}$, output channel $C_{o}$, kernel size $k$, stride size $s$, dilation size $d$, and padding size $d$ are listed. $-$ denotes no value. Each layer is followed by a batch normalization layer and a ReLU activation function except the Detector and Descriptor Heads.}
\label{tab:network}
\end{table}

==> figs_tables/table_robotcar.tex <==
\setlength{\tabcolsep}{4.pt}

\begin{table}
	%\footnotesize
	%\tiny
	\scriptsize
	\centering
		\begin{tabular}{lccc}
			\toprule
			Method & night all & night rain	& day all \\
			%\hline 
			%\hline
			\midrule
			%NV~\cite{netvlad} & 0.3 / 2.3 / 15.9 & 0.5 / 2.7 / 16.4& 6.4 / 26.3 / 90.9  \\
			%DV~\cite{densevlad} & 1.0 / 4.4 / 22.7 & 1.1 / 5.5 / 25.5 & 7.6 / 31.2 / 91.2 \\
			AS~\cite{as} & 6.9 / 15.6 / 31.7 & 7.5 / 20.0 / 35.0 &	50.9 / 80.2 / 96.6  \\
			CSL~\cite{csl} & 0.6 / 2.6 / 7.2 & 0.9 / 4.3 / 9.1  & 45.3 / 73.5 / 90.1 \\
			LLN~\cite{lln} & 13.8 / 30.3 / 57.7 & 15.7 / 34.5 / 60.5& 51.1 / 77.7 / 92.3\\
			SMC~\cite{smc} & 7.1 / 22.4 / 45.3 & 8.0 / 26.4 / 46.4	& 50.3 / 79.3 / 95.2 \\
			%AHM~\cite{ahm2019} & 22.3 / 61.8 / 94.5 & 28.4 / 68.4 / 95.5 & 45.7 / 78.0 / 95.1 \\
			SIFT~\cite{sift} & 8.7 / 14.2 / 19.6 & 9.5 / 14.5 / 17.0 & 53.5 / 77.6 / 92.6 \\
			SPP~\cite{superpoint} & 19.5 / 43.3 / 69.7 & 22.0 / 45.0 / 68.0  & 56.5 / 81.5 / 97.1 \\
			D2-Net~\cite{d2-net} & 20.4 / 40.1 / 55.0 & 22.7 / 40.5 / 56.1 & 54.5 / 80.0 / 95.3 \\
			R2D2~\cite{r2d2} & 23.7 / 46.8 / 68.0 & 29.1 / 50.2 / 68.2  & \textbf{57.4} / \textbf{81.9} / \textbf{97.9} \\
			Ours (128) & \textbf{28.0} / \textbf{54.2} / \textbf{77.3} & \textbf{34.1} / \textbf{55.0} / \textbf{76.6} & 57.2 / \textbf{81.9} / \textbf{97.9} \\
			%Ours (32) & 23.5 / 47.6 / 68.5 & 29.5 / 48.0 / 66.6 & 57.3 / 81.8 / \textbf{97.9} \\
			Ours (32) & 24.3 / 48.9 / 72.7 & 30.0 / 51.4 / 72.0 & \textbf{57.4} / \textbf{81.9} / 97.5 \\
			\bottomrule
		\end{tabular}
\caption{\textbf{Localization accuracy on the RobotCar-Seasons dataset.} The best results are highlighted.}
\label{tab:robotcar}
\end{table}

==> figs_tables/table_robotcar_4.tex <==
\setlength{\tabcolsep}{1.pt}

\begin{table}
	%\footnotesize
	%\tiny
	\scriptsize
	\centering
	\begin{center}
		\begin{tabular}{lcccc}
			Method & night all & night rain	& sun & day all \\
			%\hline 
			%\hline
			\toprule
			NV~\cite{netvlad} & 0.3 / 2.3 / 15.9 & 0.5 / 2.7 / 16.4 & 	5.7 / 16.5 / 86.7  & 6.4 / 26.3 / 90.9  \\
			DV~\cite{densevlad} & 1.0 / 4.4 / 22.7 & 1.1 / 5.5 / 25.5 & 5.7 / 16.3 / 80.2 & 7.6 / 31.2 / 91.2 \\
			AS~\cite{as} & 6.9 / 15.6 / 31.7 & 7.5 / 20.0 / 35.0 & 43.9 / 71.3 / 93.5 &	50.9 / 80.2 / 96.6  \\
			SMC~\cite{smc} & 7.1 / 22.4 / 45.3 & 8.0 / 26.4 / 46.4	 & 46.7 / 74.6 / 95.9 & 50.3 / 79.3 / 95.2 \\
			CSL~\cite{csl} & 0.6 / 2.6 / 7.2 & 0.9 / 4.3 / 9.1 & 28.0 / 47.0 / 70.4 & 45.3 / 73.5 / 90.1 \\
			LLN~\cite{lln} & 13.8 / 30.3 / 57.7 & 15.7 / 34.5 / 60.5 & 48.0 / 71.3 / 88.3 & 51.1 / 77.7 / 92.3\\
			AHM~\cite{ahm2019} & 22.3 / 61.8 / 94.5 & 28.4 / 68.4 / 95.5 & 42.0 / 71.5 / 90.7 & 45.7 / 78.0 / 95.1 \\
			SP~\cite{superpoint} & 19.5 / 43.3 / 69.7 & 22.0 / 45.0 / 68.0 & 55.4 / 79.6 / 96.7 & 56.5 / 81.5 / 97.1 \\
			R2D2~\cite{r2d2} & 23.7 / 46.8 / 68.0 & 29.1 / 50.2 / 68.2 & 56.1 / 80.0 / 96.1 & 57.4 / 81.9 / 97.9 \\
			Ours(128) & 28.0 / 54.2 / 77.3 & 34.1 / 55.0 / 76.6 & 57.6 / 80.0 / 96.5 & 57.2 / 81.9 / 97.9 \\
			Ours(32) & 23.5 / 47.6 / 68.5 & 29.5 / 48.0 / 66.6 & 55.7 / 79.6 / 97.6 & 57.3 / 81.8 / 97.9 \\
			\bottomrule
		\end{tabular}
	\end{center}
\label{tab:robotcar}
\caption{Localization accuracy on the RobotCar-Seasons dataset. We report the percentages of successfully localized images within 3 error thresholds ($0.5m,2^\circ$, $1m,5^\circ$, and $5m,10^\circ$)}.
\end{table}

==> figs_tables/table_robotcar_full.tex <==
\setlength{\tabcolsep}{1.pt}

\begin{table*}
		\footnotesize
	%\small
	\centering
	\begin{center}
		\begin{tabular}{cccccccccccc}
			Method & night all & night rain	 & overcast winter	& sun & rain & snow & dawn & dusk & night & day all & overcast summer\\
			%\hline 
			%\hline
			\toprule
			NetVlad~\cite{netvlad} & 0.3/2.3/15.9 & 0.5/2.7/16.4 & 2.8/25.9/92.6 &	5.7/16.5/86.7 &	9.0/35.9/96.0 &	7.0/25.2/91.8 &	6.2/22.8/82.6 &	7.4/29.7/92.9 &	0.2/1.8/15.5 & 6.4/26.3/90.9 & 6.5/29.6/95.2 \\
			DenseVlad~\cite{densevlad} & 1.0/4.4/22.7 & 1.1/5.5/25.5	& 4.1/26.7/93.3	& 5.7/16.3/80.2	 & 10.2/40.6/96.9 &	8.6/30.1/90.2 &	8.7/36.9/92.5 &	10.2/38.8/94.2 & 0.9/3.4/19.9 & 7.6/31.2/91.2 & 6.0/29.8/92.0 \\
			AS~\cite{as} & 6.9/15.6/31.7 & 7.5/20.0/35.0 & 43.1/82.1/96.7	& 43.9/71.3/93.5 & 62.7/83.4/98.6 & 58.3/85.3/96.9 & 52.6/80.1/95.9 & 57.4/83.5/95.9 &	6.4/11.2/28.3 &	50.9/80.2/96.6 & 38.7/76.2/99.1 \\
			SMC~\cite{smc} & 7.1/22.4/45.3	& 8.0/26.4/46.4	& 39.5/72.3/85.1 & 46.7/74.6/95.9 & 62.0/82.4/99.0 & 56.4/85.7/98.0	& 53.4/81.0/97.1 & 53.8/83.0/97.7 &	6.2/18.5/44.3 &	50.3/79.3/95.2 & 39.5/75.6/92.4 \\
			CSL~\cite{csl} & 0.6/2.6/7.2 & 0.9/4.3/9.1	& 39.5/75.9/92.3 & 28.0/47.0/70.4 &	59.9/83.1/97.6 & 53.2/83.6/92.4	& 47.2/73.3/90.1 & 56.6/82.7/95.9 & 0.2/0.9/5.3	& 45.3/73.5/90.1 & 34.1/71.1/93.5 \\
			SP+NV~\cite{superpoint} & 19.5/43.3/69.7 & 22.0/45.0/68.0 & 54.1/80.3/96.2 & 55.4/79.6/96.7	& 64.1/83.8/98.3 & 62.8/85.5/96.9 & 54.9/80.1/96.3 & 61.2/83.5/95.9	& 16.9/41.6/71.5 & 56.5/81.5/97.1 & 43.4/ 78.2/99.4 \\
			R2D2+VN~\cite{r2d2} & 23.7/46.8/68.0 & 29.1/50.2/68.2 & 55.4/80.3/97.7 & 56.1/80.0/96.1 & 64.4/83.8/98.6	& 63.4/86.1/98.6 & 56.5/80.7/97.5 & 60.9/83.8/97.2 & 18.3/43.4/67.8	& 57.4/81.9/97.9 & 45.6/78.8/99.8 \\
			Ours & 28.0/54.2/77.3 & 34.1/55.0/76.6 & 54.6/80.0/97.9	& 57.6/80.0/96.5 & 64.1/84.1/98.6 & 62.8/86.1/98.6 &	56.1/80.7/97.1 & 60.9/83.2/96.4 & 21.9/53.4/78.1 & 57.2/81.9/97.9 & 44.5/78.8/99.8\\
			
			
			\bottomrule
		\end{tabular}
	\end{center}
\label{tab:robotcar}
\caption{Localization accuracy on the RobotCar-Seasons dataset. We report the percentages of successfully localized images within 3 error thresholds ($0.5m,2^\circ$, $1m,5^\circ$, and $5m,10^\circ$)}.
\end{table*}

==> figs_tables/table_robotcar_full_snow.tex <==
\setlength{\tabcolsep}{4.pt}

\begin{table*}
	%\footnotesize
	%\small
	\scriptsize
	%\tiny
	\centering
	\begin{tabular}{llccc|cc}
		\toprule
		\multirow{2}{*}{Group} & \multirow{2}{*}{Method} & \multicolumn{3}{c}{Day} &  \multicolumn{2}{c}{Night}\\
		& & overcast-summer & overcast-winter & snow & night & night-rain \\	
		\midrule
		
		%\multirow{3}{*}{R} & Netvlad~\cite{netvlad} & 5.8 / 28.5 / 96.3 & 2.8 / 26.7 / 93.3 & 7.2 / 24.5 / 92.2 & 0.5 / 3.2 / 37.0 & 0.9 / 5.7 / 43.2 \\
		%& AP-GEM~\cite{dir} & 3.9 / 16.6 / 82.3 & 2.8 / 18.2 / 85.4 &5.5 / 15.5 / 82.2 & 0.5 / 0.7 / 21.7 & 0.0 / 1.4 / 28.2 \\
		%& Patch-Netvlad~\cite{patchnetvlad} & 5.4 / 28.5 / 91.6 & 4.1 / 24.4 / 92.1 & 7.8 / 24.9 / 89.2 & 0.2 / 1.1 / 12.8 & 1.4 / 3.9 / 20.5\\
		%\midrule
		
		\multirow{3}{*}{C} & AS~\cite{as} & 32.8 / 74.1 / 97.8 & 37.4 / 78.7 / 94.6 & 50.5 / 81.8 / 95.5 & 1.6 / 3.9 / 10.5 & 2.0 / 10.9 / 18.0 \\
		& CSL~\cite{csl} & 34.1 / 71.1 / 93.5 & 39.5 / 75.9 / 92.3 & 53.2 / 83.6 / 92.4 & 0.2 / 0.9 / 5.3 & 0.9 / 4.3 / 9.1\\
		& CPF~\cite{cascadedfiltering}  & 36.5 / 76.5 / 97.8 & 43.1 / 78.2 / 93.6 & 54.2 / 84.9 / 95.3 &  2.3 / 6.6 / 15.3 & 4.5 / 12.3 / 18.6\\
		\midrule
		
		\multirow{5}{*}{S} & SSM~\cite{ssm} & 44.1 / \textbf{79.3} / {\color{red}99.8} & 48.5 / \textbf{81.5} / 96.2 & 60.3 / 85.7 / 96.1 &  10.0 / 23.7 / 45.4 & 14.5 / 33.2 / 47.5\\
		& VLM~\cite{lln} &  41.3 / 74.5 / 96.1 & 47.4 / 75.1 / 90.3 & 55.2 / 83.0 / 91.8 &  11.9 / 26.0 / 55.0 & 15.7 / 34.5 / 60.5\\
		& SMC~\cite{smc}  & 39.5 / 75.6 / 92.4 & 39.5 / 72.3 / 85.1 &56.4 / 85.7 / {\color{red}98.0} &  6.2 / 18.5 / 44.3 & 8.0 / 26.4 / 46.4\\
		& DASGIL-FD~\cite{dasgil} & 6.0 / 31.1 / 84.7 & 5.1 / 27.2 / 85.9 & 10.6 / 29.4 / 76.9 &  1.6 / 4.8 / 19.9 & 1.8 / 4.3 / 21.6\\
		& ToDayGAN + D2Net~\cite{todaygan, d2-net} & 40.0 / {\color{red}79.0} / 98.9 & 49.0 / 77.9 / 96.2 &  57.1 / 84.5 / 95.7 & 16.4 / 43.2 / 73.3 & 24.1 / 50.5 / 74.1 \\
		\midrule
		
		\multirow{6}{*}{H} & SIFT~\cite{sift} & 39.5 / 72.4 / 91.4 & 52.6 / 78.7 / 95.1 & 61.1 / 85.1 / 95.1 &   7.8 / 13.9 / 22.1 & 9.5 / 14.5 / 17.0\\
		& SPP~\cite{superpoint} & 43.4 / 78.2 / 99.4 & 54.1 / 80.3 / 96.2 & 62.8 / 85.5 / 96.9 &   16.9 / 41.6 / 71.5 &	22.0 / 45.0 / 68.0\\
		& D2Net~\cite{d2-net} & 40.4 / 77.3 / 98.3 & 51.8 / 78.5 / 96.2 & 60.5 / 84.5 / 94.9 &  18.0 / 39.7 / 53.9 & 22.7 / 40.5 / 56.1 \\
		& R2D2~\cite{r2d2} & \textbf{45.6} / 78.8 / {\color{red}99.8} & \textbf{55.4} / 80.3 / {\color{red}97.7} & \textbf{63.4} / {\color{red}86.1} / \textbf{98.6} &   18.3 / 43.4 / 67.8 & 29.1 / 50.2 / 68.2 \\
		%& CAPS + SIFT~\cite{caps, sift} & & & 21.9 / 54.3 / 86.8 & 27.0 / 58.9 / 85.9 \\
		& DIFL + FCL~\cite{difl} & 5.4 / 27.2 / 72.8 & 4.6 / 22.8 / 78.7 & 9.0 / 25.2 / 71.8 &  0.5 / 2.7 / 8.4 & 4.5 / 10.2 / 23.2  \\
		\midrule

		\multirow{3}{*}{M} & SPP + Superglue~\cite{superpoint, superglue} &  45.1 / {\color{red}79.0} / \textbf{100.0} & {\color{red}54.6} / 80.0 / 96.2 & 62.0 / 84.9 / \textbf{98.6} &   {\color{red}24.2} / \textbf{62.6} / {\color{red}87.4} & {\color{red}42.3} / 69.3 / {\color{red}90.2}\\
		& Pixloc~\cite{backtofeature} & 41.9 / 75.4 / 99.1 & 53.8 / 80.3 / {\color{red}97.7} & 60.9 / 84.5 / 95.7 &   16.4 / 30.8 / 75.1 & 30.7 / 49.8 / 80.5\\
		& AHM~\cite{ahm2019} & 37.8 / 74.3 / 96.8 & 42.1 / 76.2 / 96.2 & 51.9 / 83.6 / 95.7 &  16.2 / 55.3 / \textbf{93.6} & 28.4 / 68.4 / \textbf{95.5} \\
		\midrule
		& LBR~\cite{lbr} &  {\color{red}45.4} / {\color{red}79.0} / \textbf{100.0} & {\color{red}54.6} / {\color{red}80.5} / \textbf{97.9} & {\color{red}63.0} / \textbf{86.5} / \textbf{98.6} &  \textbf{24.9} / {\color{red}62.3} / 86.1	& \textbf{47.5} / \textbf{73.4} / 90.0 \\ 
									
	\midrule
	\end{tabular}
\caption{\textbf{Results on RobotCar-Seasons dataset.} The best and second best results are highlighted with \textbf{bold} and {\color{red} red} fonts.}
\label{tab:robotcar}
\end{table*}

==> figs_tables/table_robotcar_v2.tex <==
\setlength{\tabcolsep}{4.pt}

\begin{table}
	%\footnotesize
	%\tiny
	\scriptsize
	\centering
		\begin{tabular}{lccc}
			\toprule
			Method & night & night rain	& day all \\
			%\hline 
			%\hline
			\midrule
			%NV~\cite{netvlad} & 0.3 / 2.3 / 15.9 & 0.5 / 2.7 / 16.4& 6.4 / 26.3 / 90.9  \\
			%DV~\cite{densevlad} & 1.0 / 4.4 / 22.7 & 1.1 / 5.5 / 25.5 & 7.6 / 31.2 / 91.2 \\
			AS~\cite{as} & 6.4 / 11.2 / 28.3 & 7.5 / 20.0 / 35.0 &	50.9 / 80.2 / 96.6  \\
			CSL~\cite{csl} & 0.2 / 0.9 / 5.3 & 0.9 / 4.3 / 9.1  & 45.3 / 73.5 / 90.1 \\
			CPF~\cite{cpf} & 2.3 / 6.6 / 15.3 & 4.5 / 12.3 / 18.6 & 48.0 / 78.0 / 94.2\\
			\midrule
			LLN~\cite{lln} & 11.9 / 26.0 / 55.0 & 15.7 / 34.5 / 60.5& 51.1 / 77.7 / 92.3\\
			SMC~\cite{smc} & 6.2 / 18.5 / 44.3 & 8.0 / 26.4 / 46.4	& 50.3 / 79.3 / 95.2 \\
			SSM~\cite{ssm} & 10.0 / 23.7 / 45.4 & 14.5 / 33.2 / 47.5 & 54.5 / 81.6 / 96.7\\
			DASGIL-FD~\cite{dasgil} & 1.6 / 4.8 / 19.9 & 1.8 / 4.3 / 21.6 & 8.7 / 30.7 / 81.3\\
			ToDayGAN + D2Net~\cite{todaygan} & 16.4 / 43.2 / 73.3 & 24.1 / 50.5 / 74.1 & 52.2 / 80.1 / 95.9\\
			\midrule
			%AHM~\cite{ahm2019} & 22.3 / 61.8 / 94.5 & 28.4 / 68.4 / 95.5 & 45.7 / 78.0 / 95.1 \\
			SIFT~\cite{sift} & 7.8 / 13.9 / 22.1 & 9.5 / 14.5 / 17.0 & 53.5 / 77.6 / 92.6 \\
			SPP~\cite{superpoint} & 16.9 / 41.6 / 71.5 & 22.0 / 45.0 / 68.0  & 56.5 / 81.5 / 97.1 \\
			D2-Net~\cite{d2-net} & 18.0 / 39.7 / 53.9 & 22.7 / 40.5 / 56.1 & 54.5 / 80.0 / 95.3 \\
			R2D2~\cite{r2d2} & 18.3 / 43.4 / 67.8 & 29.1 / 50.2 / 68.2  & \textbf{57.4} / \textbf{81.9} / \textbf{97.9} \\
			\midrule
			Ours (128) & \textbf{21.9} / \textbf{53.4} / \textbf{78.1} & \textbf{34.1} / \textbf{55.0} / \textbf{76.6} & 57.2 / \textbf{81.9} / \textbf{97.9} \\
			%Ours (32) & 23.5 / 47.6 / 68.5 & 29.5 / 48.0 / 66.6 & 57.3 / 81.8 / \textbf{97.9} \\
			Ours (32) & 18.5 / 46.3 / 73.3 & 30.0 / 51.4 / 72.0 & \textbf{57.4} / \textbf{81.9} / 97.5 \\
			\bottomrule
		\end{tabular}
\caption{\textbf{Localization accuracy on the RobotCar-Seasons dataset.} The best results are highlighted.}
\label{tab:robotcar}
\end{table}

==> sections/Introduction-20220712.tex <==
\section{Introduction}

Visual localization is key to various applications including autonomous driving and robotics. Structure-based algorithms~\cite{as,csl,smc,ssm,hfnet,lbr} involving mapping and localization processes still dominate. However, even after several decades of research, two challenges still exist: low accuracy in changing scenarios (\eg, dynamic objects and variations of illumination and seasons) and low efficiency in large-scale scenes. To address these challenges, learning-based features~\cite{d2-net,r2d2,aslfeat,superpoint,lfnet,lift,disk,contextdesc,caps,reinforcedfeatures} are introduced to replace handcrafted features~\cite{sift, rootsift, orb}. Benefiting from training on massive augmented data~\cite{hardnet,d2-net,r2d2}, these features are more robust to appearance changes. However, extracting a large number of features indiscriminately from all objects including those which are not useful for long-term localization (\eg, sky, trees, and cars), leads to accuracy and efficiency degradation caused by redundant unstable features~\cite{fgsn,smc,ssm}. Alternatively, some works~\cite{localinstance,fgsn,smc,ssm,svl,dasgil} leverage the robustness of semantics to appearance changes by filtering keypoints from unstable objects (\eg, sky, trees) as well as semantically inconsistent matches during the detection and matching processes, respectively. Nevertheless, the filtering-based usage of semantics is fragile to segmentation errors and impairs the efficiency at test time due to the requirement of additional segmentation networks which provide semantic labels. 

\begin{figure*}[t]
	%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
	\centering
	\includegraphics[width=.95\linewidth]{images/overview8}
	\caption{\textbf{Overview of our framework.} Our model implicitly incorporates semantics into the detection and description processes with the guidance of an off-the-shelf semantic segmentation network during the training process. Semantic- and feature-aware guidance is adopted to enhance its ability of embedding semantic information. Compared with previous methods~\cite{superpoint, d2-net, r2d2} using exhaustive detection and matching, by detecting features from stable objects, \eg, building, and enhancing descriptors with semantics, our model gives more inliers and much higher inlier ratio for challenging night images. Note that we detect the same number of keypoints and use the same nearest mutual matching for all methods.}
	\label{fig:framework}
\end{figure*}

Instead, we propose to implicitly incorporate semantics into both the detection and description processes, allowing our model to extract fewer but more robust features automatically in a single network. Specifically, in the detection process, unlike most previous methods~\cite{superpoint,r2d2,d2-net,d2d,keynet} adopting exhaustive detection, we encourage our detector to favor features from robust objects (\eg, buildings and traffic lanes) and suppress those from unstable objects mentioned before. In the description process, rather than utilizing triplet loss widely used for descriptor learning~\cite{hardnet,d2-net}, we employ a semantic-aware description loss consisting of two terms: inter- and intra-class losses. The inter-class loss embeds semantics into descriptors by enforcing features with the same label to be close and those with different labels to be far. The intra-class loss, which is a soft-ranking loss~\cite{aploss}, operates on features in each class independently and differentiates these features from objects of the same label. Such use of soft-ranking loss avoids the conflict with inter-class loss and retains the diversity of features in each class. With the semantic-aware loss, our model is capable to produce semantic-aware features with stronger discriminative ability especially for a significantly smaller descriptor size. Furthermore, the implicit embedding of semantic information allows our method to avoid using additional segmentation networks at test time.

Although our network is able to incorporate semantics via semantic-aware detection and description losses, it is unable to learn semantic-aware features effectively, as the local feature network is much simpler than typical segmentation networks, \eg, DeeplabV3+~\cite{deeplab3plus}. Therefore, we adopt an additional feature-consistency loss on our encoder layers to enhance its ability of embedding semantic information. Moreover, to improve the practicability of our approach, instead of using costly to obtain ground-truth labels for training, we train our model with the output of an off-the-shelf segmentation network~\cite{deeplab3plus}, which has achieved promising performance in the scene parsing task~\cite{ade20k}, but other semantic segmentation networks could also be used such as~\cite{segnet2017}. 

An overview of our system and a testing sample are shown in Fig.~\ref{fig:framework}. We embed semantics implicitly into our network with the guidance of a segmentation network in the training process. At test time, our model produces semantic-aware features from a single network directly. We summarize contributions as follows:

\begin{itemize}
	\item We propose a novel feature network which implicitly incorporates semantics into the detection and description processes, enabling our model to produce fewer but more robust semantic-aware features directly.
	\item We adopt a combination of semantic-aware and feature-aware guidance strategy to make our model embed semantic information more effectively during the training process.
	\item Our approach outperforms previous methods consistently on both feature matching and large-scale localization tasks especially under challenging conditions and even our descriptor with 4$\times$ smaller size gives competitive results.
	%\item Our semantic-aware features can give at least comparable results as previous ones with even 4-time smaller size, making the localization system more efficient.
\end{itemize}
%Our results on HPatches~\cite{hpatches} and Visuallocalization~\cite{visuallocalization} datasets demonstrate that the proposed method outperforms previous approaches consistently.

We organize the rest of this paper as follows. In Sec.~\ref{sec:relatedworks}, we introduce related works. In Sec.~\ref{sec:method}, our method is described in detail. We discuss experiments in Sec.~\ref{sec:experiments} and conclude the paper in Sec.~\ref{sec:conclusion}.

%Instead, we propose to embed semantics into a local feature network implicitly, allowing it to learn \textit{where to detect} and \textit{how to describe}. To this end, we take full advantages of priors that different features behave diversely in the long-term localization task and focus on detecting \textit{globally reliable} features directly. By focusing on robust areas, our model is able to extract fewer but more stable features automatically. Without the distraction of unstable features, descriptors of remained ones can give more accurate matches because of the reduced searching space. Moreover, descriptors further augmented by the semantic information have stronger discriminative ability even with much smaller size, promoting the localization accuracy and efficiency. Considering the requirement of ground-truth semantic labels for training degrades the practicability, instead of relying on laboriously annotated semantic labels, we leverage off-the-shelf semantic segmentation networks~\cite{deeplab3plus, segnet2017}, which have achieved promising performance in scene parsing tasks, to guide our model for training, implicitly and explicitly.

%we train our model directly with the guidance of off-the-shelf semantic segmentation networks~\cite{deeplab3plus, segnet2017}, which have achieved promising performance in scene parsing tasks. To make the learning more effective, we devise the explicit and implicit guidance strategy.

%In this paper, we take full advantages of priors that different features behave diversely in the localization task and propose to detect \textit{globally} reliable features instead. To this end, we leverage the high-level semantic information to guide the network to learn \textit{where to detect} and \textit{how to describe}. By focusing on robust areas, our model is able to extract stable features and discard sensitive ones intentionally. Without the distraction of unstable ones, descriptors of remained features can give more accurate matches because of the narrowed searching space. Moreover, descriptors augmented by the semantic information during the learning process have stronger discriminative ability even with much smaller size. Instead of using laboriously labeled semantic labels, we train our model directly with the output of off-the-shelf semantic segmentation networks~\cite{deeplab3plus, segnet2017, pspnet2017}, which have achieved promising performance in the scene parsing task. To fully utilize the provided semantic information, we propose the explicit and implicit guidance strategy. 

%Obviously, our method is different from previous works using semantic labels to reject wrong matches~\cite{vso2018, localinstance, fgsn, localinstance, smc, ssm}. First of all, they require additional networks for semantic segmentation in real applications, which degrade the efficiency. Additionally, hard assignment of semantic labels can be heavily influenced by accuracy of segmentation, which also undergoes performance drop especially in challenging conditions. 

%As they rely on other features to establish initial correspondences, they still bear the limitations of these features. 


==> sections/Relatedworks-20220712.tex <==
\section{Related Works}
\label{sec:relatedworks}

In this section, we discuss related works about visual localization, local features, and knowledge distillation. 

\subsection{Visual Localization}
%\noindent
%\textbf{Visual Localization}
Visual localization methods can be roughly categorized as image-based and structure-based. Image-based systems recover camera poses by finding the most similar one in the database with global features, \eg, NetVLAD~\cite{netvlad}. Due to the limited number of images in the database, they can only give approximate poses. To obtain more precise poses, structure-based methods build a sparse 3D map via SfM (structure from motion) and estimate the pose via PnP (perspective-n-point) from 2D-3D correspondences~\cite{as,csl,visuallocalization,hfnet,cpf}. They rely heavily on local features and are not robust to changes of illumination, weather, and season. Since the map has to store a large number of keypoints with high-dimension descriptors, it grows in size with the scale of the scene, reducing both the memory and time efficiency. Some other works have tried to predict the camera pose directly from images, \eg, PoseNet~\cite{posenet} and its variations~\cite{glnet}, or regress scene coordinates~\cite{dsac,dsac++,localinstance,vsnet}. However, the former have been proved to perform similar to image retrieval~\cite{sattler2019understanding} and latter are hard to scale to large-scale scenes.


% With the popularity of deep learning in recent years
Suffering less from appearance changes, semantics are widely used in visual localization~\cite{fgsn,stenborg2018long,localinstance,vsnet,svl,lln,smc,ssm, dasgil}. LLN~\cite{lln} uses the discriminative landmarks for place recognition. SMC~\cite{smc}, SSM~\cite{ssm}, and DASGIL~\cite{dasgil} incorporate segmentation networks into a standard localization pipeline to reject semantically-inconsistent matches. FGSN~\cite{fgsn} integrates a fine-grained segmentation network to produce more class labels for feature matching. Unlike these methods, which are sensitive to segmentation failures and require additional models to provide explicit semantic labels for filtering, we embed the semantic information into the network and produce semantic-aware features directly from a single network. 

More recently, keypoint-~\cite{superglue, dualresolution, sparsenc, pdcnet} and pixel-based~\cite{loftr,patch2pix,conditionedmatching} matching networks have been introduced to improve the accuracy by enhancing matching robustness. They have achieved excellent improvements but at a huge cost of memory~\cite{loftr,sparsenc,dualresolution,patch2pix} and time~\cite{superglue,pdcnet,sgmnet} efficiency, while in this paper, we focus mainly on learning robust local features.
% and gives semantic-aware features at test time directly without the requirement of any auxiliary assistance.
 
%LLN~\cite{lln} utilizes the discriminative landmarks for place recognition. SMC~\cite{toft2018semantic} incorporates an additional semantic segmentation module in a standard localization pipeline to reject wrong matches which don't meet semantic consistency. FGSN~\cite{fgsn} integrates a fine-grained segmentation network to produce more semantic labels for feature matching.

\subsection{Local Features}
\label{sec:local_feature}
%\noindent
%\textbf{Local Features.} 
Handcrafted features~\cite{orb,sift,rootsift,hessian} have been investigated for decades and we refer readers a survey~\cite{matching2021} for more details and focus on learned features.


With the success of CNNs, many learned features are proposed to replace handcrafted descriptors~\cite{l2-net,hardnet,sosnet,contextdesc,logpolardesc, spacialcoding,lisrd,crossdescriptor}, detectors~\cite{keynet,d2d,llf}, or both~\cite{lift,superpoint,delf2017,lfnet,d2-net,r2d2,aslfeat,reinforcedfeatures,disk}. HardNet~\cite{hardnet} focuses on metric learning by maximizing the distance between the closest positive and negative examples. ContextDesc~\cite{contextdesc} introduces the context to enhance the ability of descriptors. CAPS~\cite{caps} breaks the limitation of requiring correspondences for training and utilizes epipolar constraint instead. LIFT~\cite{lift} is the first to predict the score map of keypoints, estimate the orientation, and compute the descriptor progressively in three branches. SuperPoint~\cite{superpoint} takes keypoint detection as a supervised task, training detector from synthetic geometric shapes. LF-Net~\cite{lfnet} estimates position, scale, and orientation of features by jointly optimizing the detector and descriptor. DISK~\cite{disk} learns feature extraction by maximizing the matching reward. D2-Net~\cite{d2-net} uses local maxima across the channels as score map. R2D2~\cite{r2d2} considers both the repeatability and reliability and utilizes the average precision loss~\cite{aploss} for descriptor training. ASLFeat~\cite{aslfeat} employs deformable convolutional networks to learn shape-aware dense features.


As they focus mainly on \textit{local reliability} of features, regardless of their promising performance in feature matching, they still suffer from a huge loss of accuracy in the long-term large-scale localization task. To increase the efficacy, these methods produce descriptors with very large size from 128~\cite{r2d2,aslfeat,d2d,disk}, to 256~\cite{superpoint,lfnet}, and even 512~\cite{d2-net}, leading to low efficiency in real applications. Essentially different with these methods, our model detects and extracts \textit{globally reliable} features with the guidance of high-level semantics.  As a result, our features are able to produce more accurate matching and localization results especially under challenging conditions even with descriptor size of only 32.

\subsection{Knowledge Distillation}
Knowledge distillation techniques have been widely used for tasks including model compression~\cite{hfnet} and knowledge transfer~\cite{cross-model-knowledge}. Our usage of pseudo ground-truth local reliability and semantic labels predicted by off-the-shelf networks is more like a knowledge transfer task. In this paper, we focus mainly on how to effectively leverage the high-level semantics for low-level feature extraction.

%Instead of using explicit correspondences for supervision, CAPS~\cite{caps} utilizes camera pose for training, reducing the cost of collecting pixel-wise correspondences. During inference, these methods have to rely on other detectors to offer positions of keypints. Some works aim on detector learning. FAST~\cite{fast} was the first to detect corners with machine learning techniques. More recently, TILDE~\cite{tilde} adopts several piece-wise linear regression models to detect keypoints which are robust in various illumination and weather conditions. CDet~\cite{cdet} and TCDet~\cite{tcdet} leverage covariant features for detection. QuadNet~\cite{quadnet} uses a ranking scheme of point responses as the lost function. Key.Net~\cite{keynet} combines the handcrafted and learned CNN filters within a shallow network for scale-aware keypoints detection.

%Specially, deep neural networks have promoted the development of image semantic segmentation to a great extent and a number of methods have be proposed in the literature. Among these methods, FCN~\cite{fcn2015} is considered as a milestone, generating pixel-wise labels of arbitrary image size with a fully convolution network. ParseNet~\cite{parsenet2016}, DeepLab families~\cite{deeplabv1, deeplabv2, deeplabv3, deeplab3plus}, PSPNet~\cite{pspnet2017}, SegNet~\cite{segnet2017}, HRNet~\cite{hrnet2019}, DFANet~\cite{dfanet2019}, and many other excellent works~\cite{li2020spatial, gas2020}. We refer the readers a comprehensive survey~\cite{minaee2020image} for the whole development of image semantic segmentation.


%Most of the these methods utilize semantics to enforce pixel-wise consistency by assuming semantics are part of input. As feature detection and description is a fundamental task, in this paper, we adopt a more flexible strategy by using semantics produced by a on-the-shelf segmentation network as the auxiliary information to guide the feature detection and description implicitly and explicitly only in the training process. Our model, however, can be used individually in testing process.


